Automated Benchmark-Driven Design and Explanation of Hyperparameter Optimizers

Automated hyperparameter optimization (HPO) has gained great popularity and is an important ingredient of most automated machine learning frameworks. The process of designing HPO algorithms, however, is still an unsystematic and manual process: Limitations of prior work are identified and the improvements proposed are -- even though guided by expert knowledge -- still somewhat arbitrary. This rarely allows for gaining a holistic understanding of which algorithmic components are driving performance, and carries the risk of overlooking good algorithmic design choices. We present a principled approach to automated benchmark-driven algorithm design applied to multifidelity HPO (MF-HPO): First, we formalize a rich space of MF-HPO candidates that includes, but is not limited to common HPO algorithms, and then present a configurable framework covering this space. To find the best candidate automatically and systematically, we follow a programming-by-optimization approach and search over the space of algorithm candidates via Bayesian optimization. We challenge whether the found design choices are necessary or could be replaced by more naive and simpler ones by performing an ablation analysis. We observe that using a relatively simple configuration, in some ways simpler than established methods, performs very well as long as some critical configuration parameters have the right value.

==> latex-math/ml-bagging.tex <==
% ml - bagging, random forest

\newcommand{\bl}[1]{b^{[#1]}(\mathbf{x})}											% baselearner with argument for m
\newcommand{\blm}{\bl{m}}												    % baselearner without argument for m
\newcommand{\blmh}{\hat{b}^{[m]}(\mathbf{x})}										% estimated base learner 
\newcommand{\fM}{f^{[M]}(\mathbf{x})}                    % ensembled predictor
\newcommand{\fMh}{\hat f^{[M]}(\mathbf{x})}                    % estimated ensembled predictor
\newcommand{\ambifM}{\Delta\left(\fM\right)}          % ambiguity/instability of ensemble


==> latex-math/ml-bayesopt.tex <==
% ml - Bayesian Optimization

\newcommand{\minit}{m_{\text{init}}											% Size of the initial design
\newcommand{\lambdai}{\lambda^{[i]}											% input for black box optimization 
\newcommand{\lambdaopt}{\lambda^{*}}											% Minimum of the black box function Psi
\newcommand{\metadata}{\left\{\left(\lambdai, \Psi^{[i]}\right)\right\}}		% Metadata for the Gaussian process
\newcommand{\lambdavec}{\left(\lambda^{[1]}, \dots, \lambda^{[\minit]}\right)}  % Vector of different inputs


% \newcommand{\metadata}



\newcommand{\gp}{\mathcal{GP}\left(m(x), k\left(x, x'\right)\right)} 								% Gaussian Process 


==> latex-math/ml-boosting.tex <==
% ml - boosting
\newcommand{\fm}{f^{[m]}}                                                   % prediction in iteration m
\newcommand{\fmh}{\hat{f}^{[m]}}                                            % prediction in iteration m
\newcommand{\fmd}{f^{[m-1]}}                                                % prediction m-1
\newcommand{\fmdh}{\hat{f}^{[m-1]}}                                         % prediction m-1
\newcommand{\bmm}{b^{[m]}}                                                  % basemodel m
\newcommand{\bmmxth}{b(\mathbf{x},\bm{\theta}^{[m]})}                           % basemodel of x and theta m
\newcommand{\bmmh}{\hat{b}^{[m]}}                                           % basemodel m with hat
\newcommand{\betam}{\beta^{[m]}}                                            % weight of basemodel m
\newcommand{\betamh}{\hat{\beta}^{[m]}}                                     % weight of basemodel m with hat
\newcommand{\betai}[1]{\beta^{[#1]}}                                        % weight of basemodel with argument for m
\newcommand{\errm}{\text{err}^{[m]}}                                        % weighted in-sample misclassification rate
\newcommand{\wm}{w^{[m]}}                                                   % weight vector of basemodel m
\newcommand{\wmi}{w^{[m](i)}}                                               % weight of obs i of basemodel m
\newcommand{\thetam}{\bm \theta^{[m]}}                                    % parameters of basemodel m
\newcommand{\thetamh}{\hat{\bm \theta}^{[m]}}                             % parameters of basemodel m with hat
\newcommand{\rmm}{\tilde{r}^{[m]}}                                                  % pseudo residuals
\newcommand{\rmi}{\tilde{r}^{[m](i)}}                                               % pseudo residuals
\newcommand{\Rtm}{R_{t}^{[m]}}                                              % terminal-region
\newcommand{\Tm}{T^{[m]}}                                                   %
\newcommand{\ctm}{c_t^{[m]}}                                                % mean, terminal-regions
\newcommand{\ctmh}{\hat{c}_t^{[m]}}                                         % mean, terminal-regions with hat
\newcommand{\ctmt}{\tilde{c}_t^{[m]}}                                       % mean, terminal-regions
\newcommand{\fxk}{f_k(x)}                                                   % f_k(x)
\newcommand{\Lp}{L^\prime}
\newcommand{\Ldp}{L^{\prime\prime}}
\newcommand{\Lpleft}{\Lp_{\text{left}}}

\newcommand{\Lxyim}{L\left(\yi, f^{[m-1]}(\xi)\right)}

==> latex-math/ml-feature-sel.tex <==
% ml - feature selection

\newcommand{\xjNull}{x_{j_0}}
\newcommand{\xjEins}{x_{j_1}}
\newcommand{\xl}{\mathbf{x}_l}
\newcommand{\pushcode}[1][1]{\hskip\dimexpr#1\algorithmicindent\relax} % IGNORE_NOTATION


==> latex-math/ml-gp.tex <==
% ml - Gaussian Process

\newcommand{\gp}{\mathcal{GP}\left(m(\bm{x}), k\left(\bm{x}, \bm{x}^\prime\right)\right)} 								% Gaussian Process Definition	
\newcommand{\mvec}{\mathbf{m}}												    						% Gaussian process mean vector
\newcommand{\Kmat}{\mathbf{K}}																			% estimated base learner 
\newcommand{\ls}{\ell}                                           % length-scale


==> latex-math/ml-interpretable.tex <==


%%%%%% marginalized functions
\newcommand{\fj}{f_j}                                           % marginal function f_j, depending on feature j
\newcommand{\fnj}{f_{-j}}                                       % marginal function f_{-j}, depending on all features but j
\newcommand{\fS}{f_S}                                           % marginal function f_S depending on feature set S
\newcommand{\fC}{f_C}                                           % marginal function f_C depending on feature set C
\newcommand{\fhj}{\fh_j}                                        % marginal function fh_j, depending on feature j
\newcommand{\fhnj}{\fh_{-j}}                                    % marginal function fh_{-j}, depending on all features but j
\newcommand{\fhS}{\fh_S}                                        % marginal function fh_S depending on feature set S
\newcommand{\fhC}{\fh_C}                                        % marginal function fh_C depending on feature set C


\newcommand{\XSmat}{\Xmat_S}                                    % Design matrix subset
\newcommand{\XCmat}{\Xmat_C}                                    % Design matrix subset
\newcommand{\Xnj}{\Xmat_{-j}}                                   % Design matrix subset -j = {1, .., j-1, j+1, ..., p}
%%%%% Shapley values
\newcommand{\Scupj}{S \cup \{j\}}                               % coalition S but without player j
\newcommand{\Scupk}{S \cup \{k\}}                               % coalition S but without player k
\newcommand{\SsubP}{S \subseteq P}                              % coalition S subset of P
\newcommand{\SsubPnoj}{\SsubP \setminus \{j\}}                  % coalition S subset of P without player j
\newcommand{\SsubPnojk}{\SsubP \setminus \{j,k\}}               % coalition S subset of P without player k
\newcommand{\phiij}{\hat{\phi}_j^{(i)}}                         % Shapley value for feature j and observation i


%%%%% LIME 
\newcommand{\Gspace}{\mathcal{G}}								% Hypothesis space for surrogate model
\newcommand{\neigh}{\phi_{\xv}}									% Proximity measure
\newcommand{\zv}{\mathbf{z}}									% Sampled datapoints for surrogate
\newcommand{\Zspace}{\mathcal{Z}}								% Space of sampled datapoints
\newcommand{\Gower}{d_G}										% Gower distance



==> latex-math/ml-lm.tex <==
\newcommand{\thx}{\thetab^T \xv}												% linear score: theta^T x



==> latex-math/ml-nn.tex <==
% ml - NNs
\newcommand{\neurons}{z_1,\dots,z_M} % vector of neurons

\newcommand{\hidz}{\mathbf{z}}                            % vector of hidden activations
\newcommand{\biasb}{\mathbf{b}}                           % bias vector

\newcommand{\biasc}{c}                          % bias in output


\newcommand{\wtw}{\mathbf{w}}                             % weight vector (general)

\newcommand{\Wmat}{\mathbf{W}}                             % weight vector (general)


\newcommand{\wtu}{\mathbf{u}}                             % weight vector of output neuron
%


% deeplearning - regularization
\newcommand{\Oreg}{\mathnormal{R}_{reg}(\theta|X,y)}				% regularized objective function
\newcommand{\Ounreg}{\mathnormal{R}_{emp}(\theta|X,y)}			% unconstrained objective function
\newcommand{\Pen}{\Omega(\theta)}							% penalty
\newcommand{\Oregweight}{\mathnormal{R}_{reg}(w|X,y)}			% regularized objective function with weight 
\newcommand{\Oweight}{\mathnormal{R}_{emp}(w|X,y)}				% unconstrained objective function with weight
\newcommand{\Oweighti}{\mathnormal{R}_{emp}(w_i|X,y)}			% unconstrained objective function with weight w_i
\newcommand{\Oweightopt}{\mathnormal{J}(w^*|X,y)}				% unconstrained objective function withoptimal  weight
\newcommand{\Oopt}{\hat{\mathnormal{J}}(\theta|X,y)}				% optimal objective function 
\newcommand{\Odropout}{\mathnormal{J}(\theta, \mu|X,y)}	           	% dropout objective function

% deeplearning - optimization
\newcommand{\Loss}{L(y, f(\xv, \thetab))}
\newcommand{\Lmomentumnest}{L(\yi, f(x^{(i)}, \thetab + \varphi \nub))}                  % momentum risk
\newcommand{\Lmomentumtilde}{L(\yi, f(x^{(i)}, \tilde{\thetab}))}                  % Nesterov momentum risk
\newcommand{\Lmomentum}{L(\yi, f(x^{(i)}, \thetab))} 
\newcommand{\Hess}{\mathbf{H}}
\newcommand{\nub}{\boldsymbol{\nu}}

% deeplearning - autoencoders
\newcommand{\uauto}{L(x,g(f(x)))}			% undercomplete autoencoder objective function
\newcommand{\dauto}{L(x,g(f(\tilde{x})))}		% denoising autoencoder objective function

% deeplearning - adversarials 
\newcommand{\deltab}{\boldsymbol{\delta}}
\newcommand{\Lossdeltai}{L(\yi, f(\xi + \deltab|\thetab))}
\newcommand{\Lossdelta}{L(y, f(\xv + \deltab| \thetab))}


==> latex-math/ml-rf.tex <==
% ml -  ensemble methods, random forest

\newcommand{\betam}{\beta^{[m]}}												% baselearner with argument for m
\newcommand{\betaM}{\beta^{[M]}}												% baselearner with argument for M
\newcommand{\betai}{\beta^{[1]}}												% baselearner with argument for 1


==> latex-math/ml-survival.tex <==
\newcommand{\Ti}[1][i]{T^{(#1)}}
\newcommand{\Ci}[1][i]{C^{(#1)}}  
\newcommand{\oi}[1][i]{o^{(#1)}}  
\newcommand{\ti}[1][i]{t^{(#1)}}  
\newcommand{\lambdai}[1][i]{\lambda^{(#1)}}  
\newcommand{\deltai}[1][i]{\delta^{(#1)}}  
\newcommand{\Lxdi}{L\left(\bm{\delta}, \fx\right)}           



==> latex-math/ml-svm.tex <==
% ml - svms
\newcommand{\sv}{\operatorname{SV}}                                         % supportvectors
% already defined in basic-math:
\newcommand{\HS}{\Phi}                                               % H, hilbertspace
\renewcommand{\sl}{\zeta}
\newcommand{\slvec}{\left(\zeta^{(1)}, \zeta^{(n)}\right)}		% slack variables (SVM)
\newcommand{\sli}{\zeta^{(i)}}																% slack variable (SVM)


\newcommand{\alphah}{\hat{\alpha}}													% alpha-hat
\newcommand{\alphav}{\bm{\alpha}}													% vector alpha (bold)
\newcommand{\alphavh}{\hat{\bm{\alpha}}}													% vector alpha-hat



\newcommand{\phix}{\phi(\xv)}          												% \phi(x)
\newcommand{\phixt}{\phi(\tilde \xv)}        										% \phi(x-tilde)



==> latex-math/ml-trees.tex <==
% ml - trees, extra trees

\newcommand{\Np}{\mathcal{N}}												% (Parent) node N
\newcommand{\Npk}{\Np_k}														% node N_k
\newcommand{\Nl}{\Np_1}														% Left node N_1
\newcommand{\Nr}{\Np_2}														% Right node N_2
\newcommand{\pikN}{\pi_k^{(\Np)}}                                           		% class probability node N
\newcommand{\pikNh}[1][k]{\hat\pi_#1^{(\Np)}}                                           % estimated class probability node N
\newcommand{\pikNlh}[1][k]{\hat\pi_#1^{(\Nl)}}
\newcommand{\pikNrh}[1][k]{\hat\pi_#1^{(\Nr)}}


==> latex-math/probmodel.tex <==


% gaussians
\newcommand{\muk}{\bm{\mu_k}}  

